Layer-Stack Temperature Scaling

Recent works demonstrate that early layers in a neural network contain useful information for prediction. Inspired by this, we show that extending temperature scaling across all layers improves both calibration and accuracy. We call this procedure "layer-stack temperature scaling" (LATES). Informally, LATES grants each layer a weighted vote during inference. We evaluate it on five popular convolutional neural network architectures both in- and out-of-distribution and observe a consistent improvement over temperature scaling in terms of accuracy, calibration, and AUC. All conclusions are supported by comprehensive statistical analyses. Since LATES neither retrains the architecture nor introduces many more parameters, its advantages can be reaped without requiring additional data beyond what is used in temperature scaling. Finally, we show that combining LATES with Monte Carlo Dropout matches state-of-the-art results on CIFAR10/100.

==> files/cifar100id.tex <==
\begin{table}
\scriptsize
\caption{A comparison between LATES (abbreviated L) and temperature scaling (abbreviated T) on  CIFAR100 \cite{Krizhevsky09learningmultiple} for the five metrics: ECE, negative log-likelihood (NLL), Brier score, accuracy (ACC), and AUC. The five architectures are: {\sc vgg16} ({\sc v16}), {\sc vgg19} ({\sc v19}), {\sc resnet18} ({\sc r18}), {\sc resnet50} ({\sc r50}), and {\sc wide-resnet-28-10} ({\sc w28}).}\vspace{1mm}
\label{table:ind-cifar100}
\begin{tabularx}{\columnwidth}{@{}llXXXXX@{\hspace{0.1em}}}
\toprule
%Architecture & & \multicolumn{5}{c}{Metrics} \\ \midrule
& &
  \multicolumn{1}{c}{ECE $\downarrow$} &
  \multicolumn{1}{c}{NLL $\downarrow$} &
  \multicolumn{1}{c}{Brier $\downarrow$} &
  \multicolumn{1}{c}{ACC $\uparrow$} &
  \multicolumn{1}{c}{AUC $\uparrow$}
    \\ \midrule

\sc v16 &
  \begin{tabular}[l]{@{}l@{}} \sc t \\ \bf \sc l
    \end{tabular} & \begin{tabular}[c]{@{}c@{}}  0.04$\pm$0.00 \\  \bf 0.02$\pm$0.00 \end{tabular}&\begin{tabular}[c]{@{}c@{}} 
 1.24$\pm$0.03 \\  \bf 0.98$\pm$0.02 \end{tabular}&\begin{tabular}[c]{@{}c@{}} 
 -0.58$\pm$0.01 \\   \bf -0.63$\pm$0.01 \end{tabular}&\begin{tabular}[c]{@{}c@{}}  0.70$\pm$0.01 \\  \bf 0.73$\pm$0.01 \end{tabular}&\begin{tabular}[c]{@{}c@{}} 0.97$\pm$0.00 \\  \bf 0.98$\pm$0.00 \end{tabular} \\ \midrule\sc v19 &
  \begin{tabular}[l]{@{}l@{}} \sc t \\ \bf \sc l
    \end{tabular} & \begin{tabular}[c]{@{}c@{}}  0.05$\pm$0.01 \\ \bf 0.03$\pm$0.00 \end{tabular}&\begin{tabular}[c]{@{}c@{}}   1.30$\pm$0.02 \\   \bf 0.97$\pm$0.02 \end{tabular}&\begin{tabular}[c]{@{}c@{}}   -0.58$\pm$0.01 \\  \bf -0.63$\pm$0.01 \end{tabular}&\begin{tabular}[c]{@{}c@{}}  0.70$\pm$0.01 \\  \bf 0.73$\pm$0.01 \end{tabular}&\begin{tabular}[c]{@{}c@{}}  0.96$\pm$0.00 \\  \bf 0.99$\pm$0.00 \end{tabular} \\ \midrule\sc r18 &
  \begin{tabular}[l]{@{}l@{}} \sc t\\ \bf \sc l
    \end{tabular} & \begin{tabular}[c]{@{}c@{}}  0.04$\pm$0.00  \\ \bf 0.02$\pm$0.00 \end{tabular}&\begin{tabular}[c]{@{}c@{}}  1.05$\pm$0.03 \\  \bf 0.92$\pm$0.02 \end{tabular}&\begin{tabular}[c]{@{}c@{}}   -0.63$\pm$0.01 \\   \bf -0.65$\pm$0.01 \end{tabular}&\begin{tabular}[c]{@{}c@{}}  0.73$\pm$0.01 \\  \bf 0.75$\pm$0.01 \end{tabular}&\begin{tabular}[c]{@{}c@{}}  0.98$\pm$0.00 \\   \bf 0.99$\pm$0.00 \end{tabular} \\ \midrule\sc r50 &
  \begin{tabular}[l]{@{}l@{}} \sc t \\ \bf \sc l
    \end{tabular} & \begin{tabular}[c]{@{}c@{}}  \bf 0.02$\pm$0.00 \\  \bf 0.02$\pm$0.00 \end{tabular}&\begin{tabular}[c]{@{}c@{}} 0.97$\pm$0.02 \\   \bf 0.95$\pm$0.02 \end{tabular}&\begin{tabular}[c]{@{}c@{}}   -0.63$\pm$0.01 \\ \bf -0.64$\pm$0.01 \end{tabular}&\begin{tabular}[c]{@{}c@{}} \bf 0.73$\pm$0.01 \\  \bf 0.73$\pm$0.01 \end{tabular}&\begin{tabular}[c]{@{}c@{}}  \bf 0.98$\pm$0.00  \\ \bf 0.98$\pm$0.00 \end{tabular} \\ \midrule\sc w28 &
  \begin{tabular}[l]{@{}l@{}} \sc t \\ \bf \sc l
    \end{tabular} & \begin{tabular}[c]{@{}c@{}}  \bf 0.05$\pm$0.00 \\ \bf 0.05$\pm$0.00 \end{tabular}&\begin{tabular}[c]{@{}c@{}}  \bf 0.89$\pm$0.02 \\   \bf 0.89$\pm$0.02 \end{tabular}&\begin{tabular}[c]{@{}c@{}} \bf -0.69$\pm$0.01 \\ \bf -0.69$\pm$0.01 \end{tabular}&\begin{tabular}[c]{@{}c@{}}\bf 0.79$\pm$0.00 \\  \bf 0.79$\pm$0.00 \end{tabular}&\begin{tabular}[c]{@{}c@{}}  \bf 0.98$\pm$0.00  \\ \bf 0.98$\pm$0.00 \end{tabular} \\ \bottomrule
\end{tabularx}
\end{table}

==> files/cifar10id.tex <==
\begin{table}
\scriptsize
\caption{A comparison between LATES and temperature scaling  on  CIFAR10 \cite{Krizhevsky09learningmultiple}. Consult Table \ref{table:ind-cifar100} for abbreviations.}\vspace{1mm}
\label{table:ind-cifar10}
\begin{tabularx}{\columnwidth}{@{}llXXXXX@{\hspace{0.1em}}}
\toprule
%Architecture & & \multicolumn{5}{c}{Metrics} \\ \midrule
& &
  \multicolumn{1}{c}{ECE $\downarrow$} &
  \multicolumn{1}{c}{NLL $\downarrow$} &
  \multicolumn{1}{c}{Brier $\downarrow$} &
  \multicolumn{1}{c}{ACC $\uparrow$} &
  \multicolumn{1}{c}{AUC $\uparrow$}
    \\ \midrule

\sc v16 &
  \begin{tabular}[l]{@{}l@{}} \sc t \\ \bf \sc l
    \end{tabular} & \begin{tabular}[c]{@{}c@{}}  0.03$\pm$0.00 \\  \bf 0.02$\pm$0.00 \end{tabular}&\begin{tabular}[c]{@{}c@{}}  0.26$\pm$0.01 \\  \bf 0.23$\pm$0.01 \end{tabular}&\begin{tabular}[c]{@{}c@{}}   -0.88$\pm$0.00 \\   \bf -0.89$\pm$0.00 \end{tabular}&\begin{tabular}[c]{@{}c@{}}   \bf 0.93$\pm$0.00 \\  \bf 0.93$\pm$0.00 \end{tabular}&\begin{tabular}[c]{@{}c@{}}  \bf 0.99$\pm$0.00 \\  \bf 0.99$\pm$0.00 \end{tabular} \\ \midrule\sc v19 &
  \begin{tabular}[l]{@{}l@{}} \sc t \\ \bf \sc l
    \end{tabular} & \begin{tabular}[c]{@{}c@{}}  0.02$\pm$0.00 \\ \bf 0.02$\pm$0.00 \end{tabular}&\begin{tabular}[c]{@{}c@{}}  0.27$\pm$0.01 \\   \bf 0.23$\pm$0.00 \end{tabular}&\begin{tabular}[c]{@{}c@{}}   -0.88$\pm$0.00 \\  \bf -0.89$\pm$0.00 \end{tabular}&\begin{tabular}[c]{@{}c@{}}  \bf 0.93$\pm$0.00 \\  \bf 0.93$\pm$0.00 \end{tabular}&\begin{tabular}[c]{@{}c@{}}  \bf 0.99$\pm$0.00 \\  \bf 0.99$\pm$0.00 \end{tabular} \\ \midrule\sc r18 &
  \begin{tabular}[l]{@{}l@{}} \sc t\\ \bf \sc l
    \end{tabular} & \begin{tabular}[c]{@{}c@{}}  \bf 0.01$\pm$0.00  \\ \bf 0.01$\pm$0.00 \end{tabular}&\begin{tabular}[c]{@{}c@{}}  0.19$\pm$0.01 \\  \bf 0.18$\pm$0.01 \end{tabular}&\begin{tabular}[c]{@{}c@{}}   \bf -0.91$\pm$0.00 \\   \bf -0.91$\pm$0.00 \end{tabular}&\begin{tabular}[c]{@{}c@{}}  \bf 0.94$\pm$0.00 \\  \bf 0.94$\pm$0.00 \end{tabular}&\begin{tabular}[c]{@{}c@{}} 0.99$\pm$0.00 \\   \bf 0.99$\pm$0.00 \end{tabular} \\ \midrule\sc r50 &
  \begin{tabular}[l]{@{}l@{}} \sc t \\ \bf \sc l
    \end{tabular} & \begin{tabular}[c]{@{}c@{}}  \bf 0.01$\pm$0.00 \\  \bf 0.01$\pm$0.00 \end{tabular}&\begin{tabular}[c]{@{}c@{}}   0.19$\pm$0.01 \\   \bf 0.19$\pm$0.01 \end{tabular}&\begin{tabular}[c]{@{}c@{}}   -0.91$\pm$0.00 \\ \bf -0.91$\pm$0.00 \end{tabular}&\begin{tabular}[c]{@{}c@{}} \bf 0.94$\pm$0.00 \\  \bf 0.94$\pm$0.00 \end{tabular}&\begin{tabular}[c]{@{}c@{}}  \bf 0.99$\pm$0.00  \\ \bf 0.99$\pm$0.00 \end{tabular} \\ \midrule\sc w28 &
  \begin{tabular}[l]{@{}l@{}} \sc t \\ \bf \sc l
    \end{tabular} & \begin{tabular}[c]{@{}c@{}}  \bf 0.01$\pm$0.00 \\ \bf 0.01$\pm$0.00 \end{tabular}&\begin{tabular}[c]{@{}c@{}}  \bf 0.15$\pm$0.00 \\   \bf 0.15$\pm$0.00 \end{tabular}&\begin{tabular}[c]{@{}c@{}} \bf -0.93$\pm$0.00 \\ \bf -0.93$\pm$0.00 \end{tabular}&\begin{tabular}[c]{@{}c@{}} \bf 0.96$\pm$0.00 \\  \bf 0.96$\pm$0.00 \end{tabular}&\begin{tabular}[c]{@{}c@{}}\bf 0.99$\pm$0.00  \\ \bf 0.99$\pm$0.00 \end{tabular} \\ \bottomrule
\end{tabularx}
\end{table}
